ORCAS-I: Queries Annotated with Intent using Weak Supervision

User intent classification is an important task in information retrieval. In this work, we introduce a revised taxonomy of user intent. We take the widely used differentiation between navigational, transactional and informational queries as a starting point, and identify three different sub-classes for the informational queries: instrumental, factual and abstain. The resulting classification of user queries is more fine-grained, reaches a high level of consistency between annotators, and can serve as the basis for an effective automatic classification process. The newly introduced categories help distinguish between types of queries that a retrieval system could act upon, for example by prioritizing different types of results in the ranking.We have used a weak supervision approach based on Snorkel to annotate the ORCAS dataset according to our new user intent taxonomy, utilising established heuristics and keywords to construct rules for the prediction of the intent category. We then present a series of experiments with a variety of machine learning models, using the labels from the weak supervision stage as training data, but find that the results produced by Snorkel are not outperformed by these competing approaches and can be considered state-of-the-art. The advantage of a rule-based approach like Snorkel's is its efficient deployment in an actual system, where intent classification would be executed for every query issued. The resource released with this paper is the ORCAS-I dataset: a labelled version of the ORCAS click-based dataset of Web queries, which provides 18 million connections to 10 million distinct queries.

==> tables.tex <==
\wojciech{TODO: add UMAP plot of bert embeddings for ORCAS-gold and subset of ORCAS-I-2M (input: query + url) coloured by the intent category}


Count of queries grouped by the number of words for each intent category for manually annotated ORCAS-gold dataset and ORCAS-2M is presented in Tables \ref{tab:orcas_test_num_word_queries} and \ref{tab:orcas2M_num_word_queries} respectively. We 

\begin{table*}[]
\centering
\caption{Count of queries grouped by the number of words for each intent category for manually annotated ORCAS-gold dataset. \wojciech{We can also do 5-6 plots but they will take more space}}
\label{tab:orcas_test_num_word_queries}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccr}
\toprule
              & mean query length & \# 1 word queries & \# 2 words queries & \# 3 words queries & \# 4 words queries & \# 5+ words queries & total \\ \midrule
Navigational & 2.49 & 51 (29.8\%)               & 39 (22.8\%)                & 47 (27.5\%)                 & 17 (10.0\%)          & 17 (10.0\%)       & 171    \\
Transactional  & 3.53 & 1 (2.3\%)                & 10 (23.3\%)                 & 14 (32.6\%)                 & 5 (11.6\%)          & 13 (30.2\%)      & 43    \\
Factual    & 3.39   & 44 (12.1\%)                & 81 (22.3\%)                 & 87 (23.7\%)                 & 63 (17.4\%)              & 88 (24.2\%)    & 363    \\
Instrumental  & 4.58  & 0 (0.0\%)                & 5 (8.5\%)               & 12 (20.3\%)                & 13 (22.0\%)                 & 29 (49.2\%)     & 59    \\
Abstain    & 3.13   & 29 (8.0\%)                 & 93 (25.3\%)               & 121  (33.3\%)               & 65 (17.9\%)         & 56 (15.4\%)       & 364    \\ 
Total       & 3.21  & 125 (12.5\%)        & 228 (22.8\%)        & 281 (28.1\%)                & 163 (16.3\%)       &   203 (20.3\%) & 1,000  \\
\bottomrule
\end{tabular}%
}
\end{table*}

\begin{table*}
\centering
\caption{Accuracy of Snorkel classifier compared to other studies}
\label{tab:other_studies}
\begin{tabular}{lcccc}
\toprule
              & Number of queries in the dataset & Features& Algorithm & Accuracy \\ \midrule
Jansen et al, 2008 & 1,523,793 & queries only &rules& 74\%\\
Ashkan et al., 2009 & 800,000 & queries only&SVM& 86\% \\
Kathuria et al., 2010 & 1,874,397& queries only & k-means& 94\%\\
Figueroa., 2015 & 60,000 & queries and URLs & MaxEnt& 82.22\%\\
\textbf{Our study} & \textbf{18,823,602} & \textbf{queries and URLs} &\textbf{rules}& \textbf{90}\%\\ 
\bottomrule
\end{tabular}%
\end{table*}

\begin{table*}[]
\centering
\caption{Count of queries grouped by the number of words for each intent category for ORCAS-2M dataset annotated with Snorkel.}
\label{tab:orcas2M_num_word_queries}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccr}
\toprule
              & mean query length & \# 1 word queries & \# 2 words queries & \# 3 words queries & \# 4 words queries & \# 5+ words queries & total \\ \midrule
Navigational & 2.26 & 97526                & 84115                 & 62497                 & 30,618          & 14,854        & 289,610    \\
Transactional  & 3.92 & 72 (0.1\%)              & 9318                 & 25936                 & 23,006           & \hspace{0.3em}25,002 (30.0\%)      & 83,334    \\
Factual    & 3.49   & 68615 (9.7\%)               & 159266 (22.5\%)                & 169006 (23.9\%)                 & 130,313 (18.4\%)              & 179,707 (25.4\%)    & 706,907    \\
Instrumental  & 4.34  & 2087  (1.8\%)               & 15651 (13.4\%)               & 24026 (20.5\%)                & 23,526 (20.2\%)                 & 51,195 (43.9\%)    & 116,485    \\
Abstain    & 3.17   & 57661                 & 209035                & 253633                 & 160,849          & 122,486        & 803,664    \\ 
Total       & 3.25  & 225961 (11.3\%)        & 477385 (23.9\%)        & 535098 (26.8\%)                & 368,312 (18.4\%)       &   393244 (19.7\%) & 2,000,000  \\
\bottomrule
\end{tabular}%
}
\end{table*}

Mean Levenshtein distance between query and url for each intent category for all three datasets can be found in Table \ref{tab:levenshtein}. 



\begin{table*}[h]
\caption{Mean Levenshtein distance between query and url for each intent category for all three datasets. We distinguish between ORCAS-I-gold annotated manually and annotated by Snorkel to see if there would be any significant differences between the labellings.}
\label{tab:levenshtein}
\begin{tabular}{@{}lcccc@{}}
\toprule
            %   & ORCAS-I-gold & ORCAS-I-gold snorkel & ORCAS-I-2M & ORCAS-I-full \\ \midrule
              & ORCAS-I-gold & \begin{tabular}[c]{@{}c@{}}ORCAS-I-gold\\ /snorkel/\end{tabular} & ORCAS-I-2M & ORCAS-I-full \\ \midrule
Navigational  & 28.85      &  29.25                                                              & 28.60    & 28.61      \\
Transactional & 40.81      &     44.16                                                           & 40.93    & 40.86      \\
Factual       & 42.61      &  43.04                                                              & 44.30    & 44.31      \\
Instrumental  & 58.15      &  58.64                                                              & 51.95    & 51.94      \\
Abstain       & 48.09      & 46.39                                                             & 46.88    & 46.88      \\ \midrule
  & 43.09      &    43.09                                                            & 43.37    & xx.xx      \\  \bottomrule
\end{tabular}
\end{table*}

